Bipartite entanglement and the arrow of time

We provide a new perspective on the close relationship between entanglement and time. Our main focus is on bipartite entanglement, where this connection is foreshadowed both in the positive partial transpose criterion due to Peres [A. Peres, Phys. Rev. Lett., 77, 1413 (1996)] and in the classification of quantum within more general non-signalling bipartite correlations [M. Frembs and A. D\"oring, arXiv:2204.11471]. Extracting the relevant common features, we identify a necessary and sufficient condition for bipartite entanglement in terms of a compatibility condition with respect to time orientations in local observable algebras, which express the dynamics in the respective subsystems. We discuss the relevance of the latter in the broader context of von Neumann algebras and the thermodynamical notion of time naturally arising within the latter.

==> Addita/AlfsenShultz.tex <==
\begin{theorem}\label{thm: Alfsen-Shultz}
    \textbf{\emph{(Alfsen-Shultz \cite{AlfsenShultz1998})}} \mf{If $\JN = (\cN_\mathrm{sa}, \{\cdot,\cdot\})$ is the JBW-algebra associated with the self-adjoint part of a von Neumann algebra $\cN$, then every order derivation on $\JN$ is of the form
    \begin{equation*}
        \delta_a: \JN \rightarrow \JN, \quad \delta_a(b) := \frac{1}{2}(ab + ba^*)
    \end{equation*}
    for some $a \in \cN$. An order derivation is self-adjoint if and only if $\delta = \delta_a$ for some self-adjoint $a \in \cN_\mathrm{sa}$ and is skew-adjoint if and only if $\delta = \delta_{ia} = \frac{i}{2}[a,\underline{\ \ }]$for some $a \in \cN_\mathrm{sa}$.}
\end{theorem}
%\mf{In the case of JW algebras this identification takes the form of a choice of involution on the complexified algebra $\JN$.}
%\mf{Note that in the case of $\JN$ this identification can be made in terms of a linear map $\delta: \cN_\mathrm{sa} \ra \cN_\mathrm{sh}$ from self-adjoint to skew-Hermitian elements given by $\delta(a) = \pm ia$. We then define $ab := \frac{1}{2}\{a,b\} + \frac{1}{2}[\delta{a},{b}]$}\footnote{More generally, one can ask when a JBW-algebra arises as the self-adjoint part of a von Neumann algebras. In \cite{AlfsenShultz_StateSpaceOfOperatorAlgebras}, Alfsen and Shultz show that a necessary and sufficient condition is the the existence of a \emph{dynamical correspondence}, roughly a map that establishes a correspondence between the self-adjoint elements of $\cN$ and generators of symmetries in the Lie algebra of skew-Hermitian elements in $\cN$ (cf. \cite{Baez2020}).}

==> Addita/ComplexStructure.tex <==
\mf{An equivalent way of putting this is the following.} Recall that $\cJ(\cA)$ is the complexification of a real algebra. We would like to extend this to a complex structure on $\cJ(\cA)$ by defining $S(a) = a_1 - ia_2$ for $a = a_1 + ia_2$ with $a_1,a_2 \in \cJ(\cA)$. By symmetry, this is consistent with the anti-commutator,
\begin{equation*}
    a \circ b^* = (a_1 \circ b_1 + a_2 \circ b_2) + i(a_2 \circ b_1 - a_1 \circ b_2)\; ,
\end{equation*}
hence, $\re(a \circ b^*) = a\circ b^* + a^* \circ b$ and $\im(a \circ b) = (a_2 \circ b_1 - a_1 \circ b_2)$,  which is consistent with
\begin{align*}
    2\re(a \circ b^*) &= (a \circ b^*) + (a \circ b^*)^* = (a \circ b^*) + (b \circ a^*)
    %= (a_1 \circ b_1 + a_2 \circ b_2) + i(a_2 \circ b_1 - a_1 \circ b_2) + (b_1 \circ a_1 + b_2 \circ a_2) + i(b_2 \circ a_1 - b_1 \circ a_2)\\
    = (a_1 \circ b_1 + a_2 \circ b_2)\; ,\\
    2\im(a \circ b^*) &= (a \circ b^*) - (a \circ b^*)^* = (a \circ b^*) - (b \circ a^*)
    %= (a_1 \circ b_1 + a_2 \circ b_2) + i(a_2 \circ b_1 - a_1 \circ b_2) - (b_1 \circ a_1 + b_2 \circ a_2) - i(b_2 \circ a_1 - b_1 \circ a_2)\\
    = (a_1 \circ b_2 - a_2 \circ b_1)\; .
\end{align*}
In particular, note that $\re(a \circ b) = \re(a)\circ\re(b) - \im(a)\circ\im(b)$ and $\im(a \circ b) = \re(a)\circ\im(b) + \im(a)\circ\re(b)$ as well as $\re(a\circ b)^* = \re(a\circ b)$ and $\im(a\circ b)^* = -\im(a\circ b)$\\

Now assume that we can extend this to an associative product such that $a \circ b = \{a,b\}$. In particular, note that for $a,b \in \cJ(\cA)$ one has
\begin{align*}
    \{a,b\} + \{a,b\}^* &= 2\{a,b\} & [a,b] + [a,b]^* &= 0\\
    \{a,b\} - \{a,b\}^* &= 0 & [a,b] - [a,b]^* &= 2[a,b]\; .
\end{align*}
This suggests to define a complex structure by setting $\re(ab) := \{a,b\}$ and $\im(ab) = [a,b]$. What type of complex structure does this impose on $\cA$? By $\re(ab) = \re(a)\circ\re(b) - \im(a)\circ\im(b)$ and $\im(ab) = \re(a)\circ\im(b) + \im(a)\circ\re(b)$, let $*: \cA \ra \cA$ be an involution such that $\cJ := \{a \in \cA \mid a^* = a\}$ and $\cL := \{a \in \cA \mid a^* = -a\}$. Clearly, every element $a \in A$ has a unique decomposition $a = a_1 + a_2$ for $a_1 \in \cJ$, $a_2 \in \cL$ (eigenspace decomposition of $\cA$ with respect to the linear involution $S$) and we set $\re(a) = a_1$, $\im(a) = a_2$. We compute
\begin{equation*}
    ab = (a_1b_1 + a_2b_2) + (a_1b_2 + a_2b_1)
\end{equation*}



In this case we compute
\begin{equation*}
    ab = (a_1b_1 - a_2b_2) + i(a_1b_2 + a_2b_1)\; .
\end{equation*}
Clearly, $\re(ab) = \re(a)\re(b) - \im(a)\im(b)$ and $\im(ab) = \re(a)\im(b) + \im(a)\re(b)$.

In terms of the complex structure $S$ we compute
\begin{align*}
    2\re(ab) = ab + (ab)^* &= ab + b^*a^*\\
    &= (a_1b_1 - a_2b_2) + i(a_1b_2 + a_2b_1) + (b_1a_1 - b_2a_2) - i(b_1a_2 + b_2a_1)\\
    &= (\{a_1,b_1\} - \{a_2,b_2\}) + i([a_1,b_2] + [a_2,b_1])\; ,
\end{align*}
whereas
\begin{align*}
    2\im(ab) =ab - (ab)^* &= ab - b^*a^*\\
    &= (a_1b_1 - a_2b_2) + i(a_1b_2 + a_2b_1) - (b_1a_1 - b_2a_2) + i(b_1a_2 + b_2a_1)\\
    &= ([a_1,b_1] - [a_2,b_2]) + i(\{a_1,b_2\} + \{a_2,b_1\})\; .
\end{align*}
Hence, in order for $S(\re(ab)) = \re(ab)$ and $S(\im(ab)) = -\im(ab)$, $[a,b] \in \cL$, i.e., $S([a,b]) = -[a,b]$. In other words, $S: \cA \ra \cA^\op$. Conversely, we define an orientation on $\cJ(\cA)$ to be a complex structure on $\cJ \oplus \cJ$ such that $S \circ I = -I \circ S$, $I^2 = -1$ and $[Ia,b] = [a,Ib] = I[a,b]$. Equivalently, one defines a map $\psi: \cJ \ra \cL$ such that $\psi_a(a) = 0$ and $[\psi_a,\psi_b] = -[\delta_a,\delta_b]$.\footnote{This is generic: cf. \cite{AlfsenShultz1998}.}

==> Addita/HomomorphismsIntoCommutativeAlgebras.tex <==
Note that we have obtained this splitting by using Stinespring dilation for the completely positive map $\phi$ \cite{Stinespring1955}. In particular, $\phi$ is a convex mixture $\phi(a) = \sum_i p_i \sigma_i(a) Q_i (= \int\ d\mu(B) \sigma(a,B) \tau(B)$, where $\sigma_i \in \mc{S}(\cA)$, $Q_i$ is a POVM and, crucially, the $p_i \geq 0$ can all be chosen positive.
%flag: link with QBC and contextuality?! - cf. \input{HomomorphismsIntoCommutativeAlgebras} above
On the other hand, if $\phi$ is only assumed positive we cannot conclude that such a factorisation exists. (Obviously, it exists if we relax the condition $p_i \in \C$.)

\textbf{Key question:} When does a positive map $\varphi: \cA \ra \cB$ with $\cB$ commutative split as $\varphi = \tau \circ \Phi$ where $\Phi: \cA \ra L^\infty(X,\mu)$ and $\tau: X \ra \cB_+$ a positive-operator valued measure. Clearly, this is the case for separable channels, however, this is not the case in general. \mf({Intuitively, the problem is that such measures can have classical properties, in particular, they `can be made coexistent, i.e., jointly measurable, by introducing a sufficient degree of unsharpness' (cf. \cite{Busch1991,?}), while reflecting nonclassical features at the same time - quasi-probability distributions!)}

Formally, note that we obtain a factoring for any channel by means of Bochner's theorem. (However, while classically this factoring can be chosen such that both maps are positive, quantum mechanically, only the combined map is positive?!)


\begin{theorem}
    ...
\end{theorem}

==> Addita/MarginalProblem.tex <==
\subsection{\mf{Marginal problem - future work}}\label{sec: marginal problem}
%flag: first translation of conjugation into time orientation (or even before, then use failure of necessity as criterion for matching time orientations!


\mf{use Thm.~\ref{thm: dilated PPT criterion}} ... Recall that by Gelfand duality, every \mf{unital commutative $C^*$-algebra $\cA$ - why $\mc{A}$ instead of $\mc{B}(\cK)$?} can be represented as the algebra of continuous functions $\cA \cong C^0(X)$ on a compact Hausdorff space $X$ \cite{GelfandNaimark1943}. In what follows we will restrict to von Neumann algebras. In this case Gelfand duality asserts that every commutative von Neumann algebra $\cN$ is isomorphic to $\cN \cong L^\infty(X,\mu)$ for $(X,\mu)$ a (localisable) measurable space (cf. \cite{Pavlov2020}). We can use this to obtain a factorisation $\Phi = \pi \circ \varphi$, where $\varphi: \cA \ra L^\infty(X,\mu)$ and $\pi: X \ra \mc{P}(\cB(\cK))$ is a \mf{projection-valued measure(?)}.


\mf{Note that if $\varphi$ is itself a von Neumann algebra homomorphism (in particular, if $\varphi$ is positive) [- no, always, restriction merely wrt $\Phi(\cA) \subset \mc{B}(\cK)$!]}, then we obtain a map $\phi = v^*\Phi v = v^*(\pi \circ \varphi)v = (v^*\pi v) \circ \varphi$, where $v^*\pi v: X \ra \mc{B}_+$ is a positive operator-valued measure. In other words, $\phi$ is a `measure-prepare channel', equivalently, $\rho$ is separable state (via the Choi-Jamio\l kowski isomorphism)! \mf{- add argument!}\\

Consequently, if we restrict to the subalgebra $\Phi(\cA) \subset \cB(\cK)$ \mf{- if(f?) $\Phi$ factors through an abelian algebra}, $\Phi^*$ is a $C^*$-homomorphism. \mf{(discuss relation: non-surjectivity vs mixed states)} Hence, by Lm.~\ref{lm: C* and anti-C* homo} $\Phi(\cA)$ is commutative and the above argument shows that $\phi_\rho$ corresponds with a prepare-measure channel, i.e., $\rho$ is separable. \mf{Is it obvious that this is the case for separable $\rho$? - yes, based on uniqueness of Stinespring (cf. Lm.~\ref{lm: Schroedinger-HJW for maps}) and canonical choice for $\Phi$ ...}

Since the PPT criterion is not necessary in general not every $\phi$ has such a decomposition/$\phi$ is onto. In other words, $\phi^* = v^*\Phi^* v$ need not be a Stinespring dilation for $\phi^*$, i.e., $\Phi^*$ is not necessarily a $C^*$-homomorphism.


Our analysis thus identifies this shortcoming with a 
\mf{type of marginal problem (with respect to $\cB$ vs $\cB(\cK)$?!) ...} Since $\Phi^*$ \emph{is} a $C^*$-homomorphism on the restriction $\Phi(\cA) \subset \mf{\cB'}$, the question becomes whether it admits an extension to a $C^*$-homomorphism over a (maximal?) commutative algebra in $\mf{\cB'}$.\\

It is instructive to consider the following example:
\begin{equation*}
    \begin{pmatrix}
        0 & 1 & 0 \\
        1 & 0 & 0 \\
        0 & 0 & 1
    \end{pmatrix}
\end{equation*}
Assume that $\varphi: M_3(\C) \ra M_3(\C)$ ...\\

Now this example is generic in that from $\Phi(p) = \Phi(p^2) = \Phi^2(p)$ we must have $\Phi(p) \in \{0,1\}$ for all $p \in \cP(\cA)$. \mf{Since $\Phi(p)$ can have negative eigenvalues, we generally only obtain a quasi-probability distribution.} (Under coarse-graining they become positive.)\\


\mf{Hence, the limits of the PPT criterion relate to the fact that pairs of probability distributions, corresponding to different orientations cannot always be extended to a joint probability distribution. This defines a type of marginal problem ...}\\


An obvious question is how close one can get to making $\Phi$ and $\Phi^*$ into $C^*$-homomorphisms. To see this, let $X$ denote the space of a maximal commutative subalgebra in $\cB \supseteq \Phi(\cA)$.\footnote{In other words, $\tilde{X}$ arises from $X$ via coarse-graining.} Next, assume that $\Phi$ and $\Phi^*$ have positive extensions $\Phi': \cA \times 1$ and $(\Phi^*)' \times 1$ to $X$ such that $\Phi = \int_{X/\tilde{X}} d\mu\ \Phi'(a \times 1)$, where $d\mu$ is the probability measure in $X$. Since still $\phi = \pi \circ \Phi'$ factors, this implies that $\Phi'(p^2) = \Phi^2(p)$, hence, $\Phi'$ and $(\Phi^*)'$ would be a $C^*$-homomorphisms and thus violate the assumption. Hence, no such extension exists. Moreover, the argument is independent of $X$, and independent of the Stinespring dilation? - if so, then if and only if; which reduces to positivity, whenever $\Phi$ and $\Phi^*$ are $C^*$-homomorphisms.\\


\begin{theorem}
     \mf{want (stronger version of PPT)} $\rho$ is entangled iff extension problem has no solution. \mf{[ - extension problem later, here PPT restricted to image (instead of Thm 5)?!]}
\end{theorem}


\mf{For instance, consider the following example from harmonic analysis. - (together with splitting of HVM states from \cite{FrembsBuscemi2021}) starting example for collaboration with Eric and Francesco?!}
%\input{Example-NoncommutativeHarmonicAnalysis}
\vspace{1cm}



\vspace{1cm}


\begin{theorem}
    Let $\Phi: \cA \ra \cB(\cK)$ a $C^*$-homomorphism onto a commutative $C^*$-algbera $L^\infty(X,\mu) \cong \Phi(\cA) \subset \cB(\cK)$. Then $\Phi = \pi \circ \varphi$, where $\pi: X \ra \cP(\cK)$ is a projection-valued measure and $\varphi: \cA \ra L^\infty(X,\mu)$.
\end{theorem}

%\vspace{1cm}
%\input{HomomorphismsIntoCommutativeAlgebras}
%\vspace{1cm}

\begin{proof}
    It is immediate that $\pi: X \ra \cP(\cK)$ is a projection-valued measure, since $\Phi(p) = \Phi(p^2) = \Phi(p)\Phi(p) = (\pi(\varphi(p))(\pi(\varphi(p))$, i.e., $\Phi(p) \in \cP(\cK)$ for every $p \in \cP(\cA)$. Moreover, $\Phi(0) = 0$, $\Phi(1) = 1|_{\Phi(\cA)}$, $\Phi(p+q) = \Phi(p) + \Phi(q)$ and $\Phi(pq) = \Phi(p)\Phi(q) = 0$ for all $p,q \in \cP(\cA)$ such that $pq=0$.

    Next, we consider the map $\varphi: \cA \ra L^\infty(X,\mu)$ in this factorisation. We can decompose the image of $\varphi$ in terms of the projections in $L^\infty(X,\mu)$ as $\varphi(\cA) = \int d\mu(p)\ p\varphi(\cA)p$.
    %where $p \in \mc{P}(L^\infty(X,\mu))$ a resolution of unity.
    Let $L^\infty(X',\mu') \subset \cB(\cK)$ be a maximal abelian von Neumann subalgebra containing $L^\infty(X,\mu)$. 
    
    
    
    
    \vspace{1cm}
    
    \mf{Now note that since $L^\infty(X,\mu)$ here is atomic (eq., $\mu$ is a $\sigma$-finite measure) every map $\varphi_p := p\varphi p: \cA \ra \C$ is a positive linear functional on $\cA$. What if $L^\infty(X,\mu)$ is not atomic?} Assume otherwise, then there exists $a \in \cA_+$ and $p \in \mc{P}(L^\infty(X,\mu))$ such that $\phi_p(a) < 0$. Let $|\psi\rangle \in \cK_B$ such that $|\psi\rangle\langle\psi| = \pi(p) \in \mc{P}(\cK)$, then $\langle\psi|\Phi(a)|\psi\rangle = \mathrm{tr}[p (\pi \circ \phi_p)] < 0$ contradicting positivity of $\Phi$.
    %flag: complete positivity/C^*-homomorphism enters via the decomposition into a $C^*$-homomorphism into $\varphi: \cN \ra L^\infty(X,\mu)$ - if $\phi$ was not completely positive, one only obtains a map into positive operators on $\mc{B}(\cH_B)$, which does not necessarily dilate and hence possibly not allow for an evaluation on projections, but only on positive operators, thus shielding possible negative probabilities
\end{proof}


\begin{corollary}
    The PPT criterion fails if and only if ...
\end{corollary}

\vspace{2cm}


In summary, we find that $\phi = v^*\Phi v = v^*(\pi \circ \varphi)v = (v^*\pi v) \circ \varphi$, where $v^*\pi v: X \ra \mc{B}_+$ is a \mf{positive operator-valued measure}. In other words, $\phi$ is a `measure-prepare channel', equivalently, $\rho$ is a separable state (via the Choi-Jamio\l kowski isomorphism). \mf{What about the converse: Does every measure-prepare channel have such a decomposition?!}
%flag: We compare this with Prop.~\ref{prop: PPT - pure bipartite case}, (Thm.~\ref{prop: dilated PPT criterion - bipartite, state case})}.


%\begin{proposition}\label{prop: PPT for CP maps}
    %Let $\rho \in \cS(\cH_A \otimes \cH_B)$ and let $(\Phi,v,\cK)$ be a Stinespring dilation for $\phi_\rho = v^*\Phi v$ (i.e., $v: \cH_B \ra \cK_B$ and $\Phi: \mc{B}(\cH_A) \ra \mc{B}(\cK_B)$. If $\Phi,\Phi^* \in \CPTP(\cA,\cB)$, then $\rho$ is separable.
%\end{proposition}

%\begin{proof}
    %$t(\tilde{\rho}) \in \mc{B}_+(\cH_A \otimes \cK_B)$ if and only if $\Phi_\rho \in \CPTP(\mc{B}(\cH_A),\mc{B}_+(\cK_B)) \cap \CPTP(\mc{B}(\cH_A),\mc{B}_-(\cK_B))$ by Lm.~\ref{prop: transposition vs *}, which by Lm.~\ref{lm: C* and anti-C* homo} and the preceding discussion implies that $\rho$ is separable.
%\end{proof}


%\mf{We compare this with the Prop.~\ref{prop: PPT - pure bipartite case}. By the correspondence
%\begin{equation*}
    %\rho = (\rho_{ij}) = \sum_{ij} E_{ij} \otimes \rho_{ij}
    %= \sum_{ij} E_{ij} \otimes \phi_\rho(E_{ij})
    %= \sum_{ij} E_{ij} \otimes v^*\Phi(E_{ij})v
    %= \sum_{ij} E_{ij} \otimes \tilde{\rho}_{ij}
    %= (\tilde{\rho}_{ij}) = \tilde{\rho} \; ,
%\end{equation*}
%we obtain a state $\tilde{\rho} \in \cS(\cH_A \otimes \cK_B)$. With respect to this state we obtain a sharp classification by Lm.~\ref{prop: transposition vs *}.}\\

%\textbf{Question:} Is Prop.~\ref{prop: PPT for CP maps} more general than Prop.~\ref{prop: PPT - pure bipartite case}? - pure states correspond with pure channels under the Choi-Jamio\l kowski isomorphism, i.e., channels with a single term in their Kraus representation; however, $\tilde{\rho}$ does not necessarily have to be pure?!\\

\vspace{1cm}

\textbf{Stinespring dilations. [- use after Lm.~\ref{lm: transposition vs *}?]} Let $\phi = v^*\Phi v$ be a Stinespring dilation and $\phi^* = w\Phi' w^*$ be a Stinespring dilation. When are the two dilations related?

Note that the argument is independent on the choice of Stinespring dilation.

%\mf{To see this, it is convenient to use the characterisation of completely positive maps in terms of an ancillary system. Note that in this representation one can always take the ancilla to be a pure state (cf. generalised measurements \cite{Ozawa1984}?) \mf{- think purification of state}.\\
%With this representation the independence on the choice of dilations is a consequence of Thm.~\ref{thm: Schroedinger-HJW theorem}.} \mf{More generally?}, we can translate this fact into a statement about the respective map $\phi_\rho$.


\begin{lemma}\label{lm: Schroedinger-HJW for maps}
    \mf{used before: }Let $\rho \in \cS(\cH_A \otimes \cH_B)$ and let $\phi_\rho = v_1\Phi_1 v_1^* = v_2\Phi_2 v_2^*$ be two Stinespring dilations. Then $\Phi_1^*: \cA \ra \cB$ is a $C^*$-homomorphism if and only if $\Phi_2^*: \cA \ra \cB$ is a $C^*$-homomorphism.
\end{lemma}

\begin{proof}
    %Let $(\Phi_1,v_1,\cK_1)$ and $(\Phi_2,v_2,\cK_2)$ be two Stinespring dilations for $\phi_\rho = v_1^* \Phi_1 v_1 = v_2^* \Phi_2 v_2$.
    There is a partial isometry $W: \cK_1 \ra \cK_2$ defined by $W \Phi_1 v_1 h = \Phi_2 v_2h$ for all $h \in \cH_A$ such that $\Phi_1 = W^* \Phi_2 W$.\footnote{Note that for minimal Stinespring dilations $W$ is unitary.} Hence, $\Phi^*_1 = W^* \Phi^*_2 W$ and the claim follows.
    %criterion holds with respect to the Stinespring dilation $(\Phi_1,v_1,\cK_1)$ if and only if it holds for the Stinespring dilation $(\Phi_2,v_2,\cK_2)$.
\end{proof}
%Comparing with Thm.~\ref{thm: Schroedinger-HJW theorem}, we remark that a Stinespring dilation can always be chosen such that the ancillary state is pure. \mf{From this and Eq.~(\ref{eq: channel-state duality}) it follows that $\tilde{rho}$ can be chosen to be pure, namely in which case the result follows directly from Thm.~\ref{thm: Schroedinger-HJW theorem}.}




\vspace{1cm}

In summary, entanglement is characterised by the conjugate-linear operator $S$.


\begin{theorem}\label{thm: PPT criterion - bipartite, map case}
    Let $\rho \in \cS(\cH_A \otimes \cH_B)$ and let $\phi_\rho$ the map under the isomorphism in Eq.~(\ref{eq: CJ-isomorphism}). Then $\rho$ is separable if and only if $\phi_\rho,\phi^*_\rho: \cA \ra \cB$ are completely positive \mf{(if and only if $T_1(\rho)$ positive by Lm.~\ref{lm: transposition vs *}?)} %$\Phi,\Phi^* \in \Hom(\cA,\cB)$ (equivalently, $\Phi \in \Hom(\cA,\cB) \cap \Hom(\cA,\cB^*)$), i.e., $\phi,\phi^* \in \CPTP(\cA,\cB)$.
\end{theorem}

\begin{proof}
    %flag: the argument is simply a derivation of the previous argument
    One direction is Peres' famous necessary condition for entanglement \cite{Peres1996}. To see it more directly, assume $\rho$ is separable. By Lm.~\ref{lm: transposition vs *} we obtain maps $\phi_\rho$ and $\phi_{T_1(\rho)} = \phi^*_\rho$. Let $\phi_\rho = v^*\Phi v$ be a Stinespring dilation. Since $\rho$ is separable $\Phi,\Phi^*: \cA \ra \cB(\cK)$ are $C^*$-homomorphisms by Lm.~\ref{lm: C* and anti-C* homo} \mf{(needs converse of subsequent argument)!}. It follows that $\phi^*_\rho = \phi_{T_1(\rho)}$ is completely positive by Stinespring's theorem, hence, $T_1(\rho)$ is positive by Choi's theorem.
    
    Conversely, \mf{if $T_1(\rho)$ is positive then $\phi_{T_1(\rho)} = \phi^*_\rho$ (by Lm.~\ref{lm: transposition vs *}) is completely positive by Choi's theorem.}
    Let $(\Phi,v,\cK)$ be a Stinespring dilation for $\phi_\rho$, i.e., $\phi_\rho = v^*\Phi v$. Since $\phi_\rho,\phi^*_\rho$ are completely positive, $\Phi,\Phi^*: \cA \ra \cB$ are $C^*$-homomorphisms by Stinespring's theorem \mf{- no, the dilations will generally have different $v$!}, hence, %for any Stinespring dilation of $\phi_\rho = v^*\Phi v$
    by Lm.~\ref{lm: C* and anti-C* homo} $\Phi(\cA) \subset \cB(\cK)$ is a commutative algebra. Hence, it has a factorisation into a prepare-measure channel and it follows that $\rho$ is separable. %\mf{(By Lm.~\ref{lm: Schroedinger-HJW for maps} the argument is independent of the choice of Stinespring dilation.)}
\end{proof}


\mf{\textbf{Question:} Is this version known? - at least, very similar to existing results on entanglement witnesses (generic decomposable maps? vs optimal choice of $S$); here, clarification?!}


Importantly, Thm.~\ref{thm: PPT criterion - bipartite, map case} yields an (alternative to Prop.~\ref{prop: dilated PPT criterion - bipartite, state case}) classification of separable states in terms of their representation as quantum channels. In the next section we will see how this perspective reveals an intimate correspondence between entanglement and time reversal asymmetry. \mf{(In particular, we will justify the folklore perception that the partial transpose in the homonymous entanglement criterion is closely related with time reversal.)} \mf{- add argument in Sec.~\ref{sec: } here or below?!}




%What is more, by translating the criterion to dilations we not only observe the importance of Lm.~\ref{lm: Schroedinger-HJW for maps} (/Thm.~\ref{thm: Schroedinger-HJW theorem}) in this broadly used concept, but also find the formal reason for the folklore intuition that the partial transpose corresponds with time reversal.

==> Addita/RelationWithStinespringDilations.tex <==
\mf{\textit{(Sketch:)}} We can write $\rho = \sum_i c_i |v_i\rangle\langle v_i| \otimes \rho_i$ with $\rho_i \in \cS(\cH_\cB)$, $c_i \in \C$. [Moreover, we may consider the Hilbert space $\cH_\cC$ to be part of a dilation of the system $\cB$ only.] Then the purifications are of the form $\rho_i = \tr_{\cH_\cC}[|\psi_i\rangle\langle\psi_i|]$, $|\psi_i\rangle \in \cH_\cA \otimes \cH_\cB \otimes \cH_\cC$, and we have $\rho = \sum_i |v_i\rangle\langle v_i| \otimes c_i\tr_{\cH_\cC}[|\psi_i\rangle\langle\psi_i|]$. By the Schr\"odinger-HJW theorem, there is a unitary freedom in choosing the $|\psi_i\rangle$ for every $i$. Yet, since we assumed $\rho$ to be entangled, we cannot find unitaries such that $\rho = \sum_i |v_i\rangle\langle v_i| \otimes \rho_2 = \rho_1 \otimes \rho_2$. \mf{In other words, we cannot express $|\psi_i\rangle = U_i|\psi_0\rangle$ for all $i$.} Hence, the Schmidt decomposition (with respect to $\cH_\cA$ and $\cH_B\otimes\cH_\cC$) of any purification of $\rho$ contains at least two terms, hence, it has a negative eigenvalue. \mf{Obviously, this can only be possible if $c_i \in \R$ for all $i$. In fact, the argument implies that it is impossible to find unitaries such that $c_i \in \R_+$ for all $i$---the latter case corresponding with separable states. - would need unitaries such that $c_i|\psi_i\rangle\langle\psi_i| = U_i|\psi_i\rangle\langle\psi_i|U_i^{-1}$, which is impossible (only real numbers can be produces this way)}
%flag: Note also the resemblance with the failure of the (asymptotic?!) quantum Birkhoff conjecture: not every unital CPTP map arises as a convex mixture of unitary channels (neither in terms of controls).

==> Addita/Schroedinger-HJWTheorem.tex <==
%\begin{theorem}[\mf{Schr\"odinger-HJW theorem \cite{Schroedinger1936,HughstonJoszaWootters1993}}]\label{thm: Schroedinger-HJW theorem}
    %Let $\psi \in \cS(\cN \otimes \cM)$, $\rho_\psi = \tr_{\cM}[|\psi\rangle\langle\psi|]$. Then
    %\begin{enumerate}
        %\item Every $\rho^\cN$-ensemble of order $n \leq n^{\cM}$ has a corresponding ancilla in $\cN^{\cM}$ . If the $\rho^{\cN}$-ensemble is linearly independent, the ancilla is unique.
        %\item Every orthonormal basis of $\cN \otimes \cM$ contains exactly one ancilla corresponding to exactly one $\rho^{\cN}$-ensemble.
        %\item Given any two $\rho^{\cN}$-ensembles, there exist unitary transformations on $\cN \otimes \cM$ which generate a $U$-map from one to the other; if each $\rho^{\cN}$-ensemble is linearly independent, the transformation is unique.
        %\item Every unitary transformation on $\cN \otimes \cM$ generates a $U$-map of every $\rho^{\cN}$-ensemble to another.
        %\item Every vector in the support of $\rho^{\cN}$ appears as an element of at least one $\rho^{\cN}$-ensemble .
    %\end{enumerate}
%\end{theorem}


\begin{proposition}\label{prop: dilated PPT criterion - bipartite, state case}
    Let $\rho \in \SAB$ for $\dim(\cH_\cA),\dim(\cH_\cB) \geq 2$ \mf{finite/arbitrary}. %and let $|\psi\rangle \in \cH_A\otimes \cH_B \otimes \cH_C$ be any vector such that $\rho = \tr_{\cH_C}[|\psi\rangle\langle\psi|]$.
    Then $\rho$ is separable if and only its purifications are separable \mf{for any measurement on the ancillary system}.
\end{proposition}

\begin{proof}
    Assume first that $\rho = \mathrm{tr}_{\cC}[|\psi\rangle\langle\psi|]$ such that $|\psi\rangle = \sum_i |\psi_{1,i}\rangle \otimes |\psi_{2,i}\rangle$, where $|\psi_{1,i}\rangle \in \cH_\cA \otimes \cH_{\cC_1}$ and $|\psi_{2,i}\rangle \in \cH_\cB \otimes   \cH_{\cC_2}$.\footnote{\mf{Note that this includes the cases $\cH_{\cC_1} = \C$ and/or $\cH_{\cC_2} = \C$.}} It immediately follows that $\rho$ is separable.
    
    Conversely, assume that $\rho$ is separable, i.e., it admits an ensemble decomposition of product states, $\rho = \sum_i |\phi_{\cA,i}\rangle \otimes |\phi_{\cB,i}\rangle$. \mf{Assuming the $|\phi_i\rangle$ in the ensemble decomposition $\rho = \sum_i p_i |\phi_i\rangle\langle\phi_i|$ are linearly independent (wlog?), the Schr\"odinger-HJW theorem asserts that $\rho$ has a unique purification $\rho = \mathrm{tr}_{\cC}[|\psi\rangle\langle\psi|]$, where $\cC$ is an ancillary system and $|\psi\rangle \in (\cH_\cA \otimes \cH_\cB) \otimes \cH_\cC$.} Moreover, two purifications with respect to different ensemble decompositions of $\rho$ are related by a unique unitary transformation on the ancillary system, $U = 1_\cA \otimes 1_\cB \otimes U_\cC$. It follows that $|\psi'\rangle = U|\psi\rangle$ is a product state with respect to the decomposition $\cH_\cA \otimes (\cH_\cB \otimes \cH_\cC)$ if and only if $|\psi\rangle$ is. Since we can easily find a separable purification $|\psi\rangle = |\psi_1\rangle \otimes |\psi_2\rangle$, where $|\psi_1\rangle \in \cH_\cA$ and $|\psi_2\rangle \in \cH_\cB \otimes \cH_\cC$,\footnote{\mf{In particular, we may thus consider $\cC$ as a dilation of the local system $\cB$.}} it follows that every purification $|\psi'\rangle$ of $\rho$ is separable.
    %\input{Addita/RelationWithStinespringDilations}
\end{proof}

==> Discussion/OpenQuestions.tex <==
\subsection{Open Questions}

\begin{itemize}
    \item problem of mixing
    Note that the PPT criterion derives from Prop.~\ref{prop: PPT for CP maps}, yet under the coarse-graining of the dilated system to the system $\cH_A \otimes \cH_B$, the sufficiency is lost (apart from simple cases \cite{Horodeckisz1996})
    \begin{corollary}\label{cor: partial PPT}
        Let $\rho \in \cS(\mc{B}(\cH_1) \otimes \mc{B}(\cH_2))$. If $t(\rho) \notin \mc{B}_+(\cH_A \otimes \cH_B)$, then $\phi_\rho \notin \CPTP(\mc{B}(\cH_1),\mc{B}_+(\cH_2)) \cap \CPTP(\mc{B}(\cH_1),\mc{B}_-(\cH_2))$.
    \end{corollary}

    \begin{proof}
        This follows immediately from Eq.~(\ref{eq: channel-state duality}) and Lm.~\ref{prop: transposition vs *}.
    \end{proof}
    Here, we showed that the converse of Cor.~\ref{cor: partial PPT} can be held up, together with its intrinsic interpretation of consistency with local time reversal, when lifted to dilated systems. Of course, this leaves open the related problem of classifying the types of mixtures occuring under the coarse-graining process from Thm.~\ref{thm: PPT criterion - bipartite, map case} to Prop.~\ref{prop: PPT for CP maps}! - comparison with QBC?!
    %flag: reverse convex mixtures allow for classically correlated states, i.e., mixtures of separable states?!
    
    \item since the separability problem is known to be hard in general, we conclude that this hardness lies in finding a dilation
    \begin{corollary}
        The PPT criterion is necessary and sufficient when reduced to ...
    \end{corollary}
    
    \item is this the reason for the complications arising with distillation \cite{Horodeckisz1998}?
    
    \item compare with hardness results ([Gurvits2003]): hardness to find ancilla?!
    
    \item distillability [ - and bound entanglement?!]
\end{itemize}

==> Discussion/Outlook.tex <==
\subsection{Outlook}

\subsubsection{Multipartite case - future work}

\textbf{key idea:} use all bi-partitions (restrict to separable vs entangled classification!)



\subsubsection{Stinespring dilations - future work}\label{sec: Stinespring dilations}

The discrepancy between the PPT criterion and the criterion suggested here is when $\phi^*$ has a Stinespring dilation not related by an isometry to $\phi = v^*\Phi v$. (see also marginal problem?)

\begin{itemize}
    \item Does this help to study bound entanglement?
    \item QBC (unital CPTP channels vs mixed unitary channels): study factorisation via commutative algebra (but with $\varphi: \cN \ra X$ not necessarily (having a dilation to) a homomorphism)
\end{itemize}



\subsubsection{Marginal problem - future work}\label{sec: marginal problem}
%\input{MarginalProblem}



\subsubsection{\mf{General vN algebras, TTT, (and `thermal time hypothesis'?)  - future work?}}

we have introduced time orientations somewhat externally (as additional data to the mere Jordan structure); instead, one can speculate whether the result can be interpreted in a more intrinsic way: entangled states defining a relative time orientation between subsystems ...
%NB: Note that a global time-orientation is fixed by the global von Neumann algebra $\cN$. In AQFT, $\cN$ arises as the direct limit of local algebras. As such, the flow of time on von Neumann algebras is determined by the orientations locally. In turn, without specifying such orientations, one is forced to consider nets of Jordan algebras.
%NB: The formalism of AQFT seems too rigid in defining nets of algebras on top of a given spacetime structure. Instead, the internal flow of time in von Neumann algebras suggests that the latter should arise within the algebraic setting. This puts the following challenge: identify the Lorentz/Poincare group as the group of internal symmetries of von Neumann algebras!

==> EntanglementVSTime/CPvsDMaps.tex <==
\mf{For simplicity, we first consider finite-dimensional matrix algebras over the complex numbers, for which the Jordan algebra is the set of Hermitian operators under the symmetric bracket or anti-commutator $\{a,b\} := \frac{1}{2}(ab + ba)$, i.e., $\cJ(\cA) = (H_n(\C),\{\cdot,\cdot\})$.}\footnote{Jordan algebras are inherently real algebras. Here, we usually consider their complexification (see below).}

One immediately asks which linear maps derive from Jordan homomorphisms, respectively, $C^*$-homomorphisms. For matrix algebras, this result is known as Choi's theorem \cite{Choi1975}. More generally, such maps are classified by Stinespring's theorem.


\begin{theorem}[Stinespring \cite{Stinespring1955}]\label{thm: Stinespring}
    Let $\cA$ be a $C^*$-algebra with a unit, let $\cH$ be a Hilbert space, and let $\mu$ be a linear function from $\cA$ to operators on $\cH$. Then a necessary and sufficient condition that $\mu$ have the form
    \begin{equation*}
        \mu(A) = V^*\rho(a)V \quad \quad \forall a \in \cA\; ,
    \end{equation*}
    where $V$ is a bounded linear transformation from $\cH$ to a Hilbert space $\cK$ and $\rho$ is a $*$-representation of $\cA$ into operators on $\cK$, is that $\mu$ be completely positive.
\end{theorem}


Complete positivity is well known as the essential property of maps (`channels') in quantum theory (see also \cite{Kraus1983,Choi1975}). For our purposes it will be necessary to relax the condition in Thm.~\ref{thm: Stinespring} to \emph{decomposable maps}, i.e., maps of the form $\mu(A) = V^*\rho(a)V$ as in Thm.~\ref{thm: Stinespring} except that $\rho$ is only requird to be a Jordan $*$-homomorphism. This leads to a relaxation of the notion of positivity to a symmetrised notion thereof.


\begin{theorem}[St\o rmer \cite{Stormer1982}]\label{thm: Stormer}
    Let $\cA$ be a $C^*$-algebra and $\phi$ a linear map of $\cA$ into $\BH$. Then $\phi$ is decomposable if and only if for all $n \in \N$ whenever $(x_{ij})$ and $(x_{ji})$ belong to $M_n(\cA)_+$ then $(\phi(x_{ij})) \in M_n(\BH)_+$.
\end{theorem}


On the level of the algebra, this symmetrisation corresponds to the fact that a Jordan algebra can be lifted to an associative algebra in two ways:\cite{AlfsenShultz1998,Kadison1951}
\begin{equation}\label{eq: two associative products}
    \cB_\pm(\mc{H}) := \{a \in \mc{J}(\mc{H}) \mid a \circ_\pm b = \frac{1}{2}\{a,b\} \pm \frac{1}{2}[a,b]\}\; .\footnote{\mf{In finite dimensions the algebras $\cB_\pm(\mc{H})$ are isomorphic. A celebrated result by Connes \cite{Connes1975} shows that this does not hold for von Neumann algebras in general. Is this correct - *-isomorphic vs opposite algebra?}}
\end{equation}
The positivity inherent to decomposable maps by Thm.~\ref{thm: Stormer} is a mixture of complete positivity with respect to the two algebras $\cB_\pm(\mc{H})$.\footnote{This general fact does not imply the special fact that in low dimensions ($2\times2$ and $2\times3$) positive maps are decomposable \cite{Woronowicz1976}.}

Note that for a fixed choice of basis, transposition changes the operator ordering, i.e., maps $\cB_+(\mc{H})$ to $\cB_-(\mc{H})$ and vice versa. This suggests to replace the basis-dependent $t$ with the basis-independent map $\cT: \cB_+(\mc{H}) \cB_-(\cH)$, which intuitively corresponds with time reversal \mf{(cf. complexification <--> involution <--> fixed point)}. In fact, we can now make this precise and apply the theory to general Jordan algebras, by expressing the additional information corresponding to the choice of associative product in Eq.~(\ref{eq: two associative products}) in terms of an \emph{orientation}.

==> TODO.tex <==
\textbf{TODO}
\begin{itemize}
    \item double check: What is $\cong$ in $\cA_\pm \cong (\cJ(\cA),\Psi/\Psi^*)$?, proof of Thm.~1; normalisation; TTT formulas
    \item notation: $\cA$
\end{itemize}

==> TheArrowOfTime/GeneralCase.tex <==
Crucially, there is a one-to-one correspondence between elements in $\cJ(\cA)$ and generators of symmetries, i.e., Jordan automorphisms, which we denote by $\sD$.\footnote{\mf{In the situation above, this correspondence is given by multiplication with $i$.}} Physically, this correspondence reflects the familiar dual role of observables, part of which finds expression in the well-known theorem by Noether (cf. \cite{Baez2020}).\footnote{\mf{In fact, this result is generic: (i) the set of (skew) order derivations $\sD(\cJ)$ of a JB(W) algebra $\cJ$ carries the structure of a Lie algebra; (ii) the existence of a (dynamical) correspondence $\psi: \cJ \ra \sD(\cJ)$ is the crucial ingredient in ensuring that an abstract JB(W) algebra derives from an (associative) $C^*$ (von Neumann) algebra \cite{AlfsenShultz1998}, equivalenly, $\psi$ defines a complex structure on $\cJ$; (iii) Wigner's theorem is a special case for factor algebras, more generally, symmetries are given by Jordan automorphisms, which in the case of von Neumann algebras decompose into a direct sum of a $C^*$ and an anti-$^*$-automorphism in every factor \cite{Kadison1951}.}}
%In a precise sense, a Jordan algebra derives from an associative algebra if it carries a dynamical correspondence: roughly, an identification between observables and generators of symmetries (see below for details). For more details on the distinction between Jordan admitting an associative structure, we refer to \cite{Hanche-OlsenStormer1984JordanOA,AlfsenShultz2001,AlfsenShultz2003}. See also \cite{Baez2020} for a recent discussion on the physical significance of this distinction.

\mf{We conclude that specifying a complex structure $S$ on $\cJ$ is equivalent to specifying the operator ordering in Eq.~(\ref{eq: two associative products}) \mf{or the sign in the commutator}.}
%\input{ComplexStructure}

\mf{Note also that this fits nicely with the fact that every anti-unitary operator is the product of a unitary operator and the time-reversal operator.}
